Why (and How) Networks Should Run Themselves

The proliferation of networked devices, systems, and applications that we depend on every day makes managing networks more important than ever. The increasing security, availability, and performance demands of these applications suggest that these increasingly difficult network management problems be solved in real time, across a complex web of interacting protocols and systems. Alas, just as the importance of network management has increased, the network has grown so complex that it is seemingly unmanageable. In this new era, network management requires a fundamentally new approach. Instead of optimizations based on closed-form analysis of individual protocols, network operators need data-driven, machine-learning-based models of end-to-end and application performance based on high-level policy goals and a holistic view of the underlying components. Instead of anomaly detection algorithms that operate on offline analysis of network traces, operators need classification and detection algorithms that can make real-time, closed-loop decisions. Networks should learn to drive themselves. This paper explores this concept, discussing how we might attain this ambitious goal by more closely coupling measurement with real-time control and by relying on learning for inference and prediction about a networked application or system, as opposed to closed-form analysis of individual protocols.

==> ml.tex <==
\section{Machine Learning}\label{sec:ml}

ML: Something on machine learning, including (i) measurement data analyzed
using machine learning, (ii) using learning to drive the
measurement/configuration of the network, (iii) doing learning (or parts of
learning) directly in the data plane [Nick]

\subsection{Real-time Inference and Analysis}

Machine learning has been applied to a wide variety of network monitoring tasks,
ranging from performance monitoring to security. For example, previous work has
incorporated network-level features into machine learning models to detect (and,
in some cases, predict) network attacks involving unwanted traffic, ranging from
denial of service attacks to Internet scams. Typically, these models use features 
that are directly observable in network traffic, such as traffic or query volume
from an individual IP address, to detect or predict an attack. 

To date, however, many of these models have been demonstrated and deployed in
a purely offline fashion: Traffic is collected from the network in the form of
packet captures, IPFIX records, or DNS query logs and is used to train a
detection model. Existing work by and large applies these models offline, as
well, collecting data from the network and applying the captured data to the
model in a separate analysis system. Yet, in practice, many of these models
are incorporate simple features---often ones that can be computed or inferred
from a single packet. Programmable switches could extract these features from
the packets in the data plane and even compute regression functions based on
these learned models, essentially computing the prediction function in-line
and making real-time decisions about the nature of traffic in the network,
without ever requiring off-path analysis.

Consider a machine-learning based spam filter, such as SNARE, which has been
developed in previous work~\cite{hao2009}. This classifier computes a score
that determines the likelihood of email traffic being spam based on features
such as the autonomous system of the sending IP address, and the number of
adjacent IP addresses that have also sent emails. Programmable switches could
easily compute these types of features inline {\em and} compute the weighted
linear combination of individual feature characteristics to compute the
overall likelihood that a message is spam. Another example involves botnet
detection based on DNS lookups: these classifiers detect abnormal features
such as lookups that are (among other features) lexicographically close
together, occur in large bursts over short time intervals, and are hosted on
authoritative DNS servers with known bad reputations. In these cases, once
again, a switch in the network could parse the DNS queries to extract these
features and detect DNS lookups associated with malicious activity in the
switches themselves, without ever requiring offline analysis.

\xxx{Could we include an apt example here, such as embedding a regression or PCA
in the data plane?}

\subsection{Using Learning to Drive Measurement}

\xxx{Active learning?}


